Single and bi-layered 2-D acoustic soft tactile skin (AST2)

This paper aims to present an innovative and cost-effective design for Acoustic Soft Tactile (AST) Skin, with the primary goal of significantly enhancing the accuracy of 2-D tactile feature estimation. The existing challenge lies in achieving precise tactile feature estimation, especially concerning contact geometry characteristics, using cost-effective solutions. We hypothesise that by harnessing acoustic energy through dedicated acoustic channels in 2 layers beneath the sensing surface and analysing amplitude modulation, we can effectively decode interactions on the sensory surface, thereby improving tactile feature estimation. Our approach involves the distinct separation of hardware components responsible for emitting and receiving acoustic signals, resulting in a modular and highly customizable skin design. Practical tests demonstrate the effectiveness of this novel design, achieving remarkable precision in estimating contact normal forces (MAE < 0.8 N), 2D contact localisation (MAE < 0.7 mm), and contact surface diameter (MAE < 0.3 mm). In conclusion, the AST skin, with its innovative design and modular architecture, successfully addresses the challenge of tactile feature estimation. The presented results showcase its ability to precisely estimate various tactile features, making it a practical and cost-effective solution for robotic applications.

==> parts/table2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[tb!]
\small\addtolength{\tabcolsep}{-4pt}
\centering
\caption{Comparison of various regression  models based on validation error for estimating contact force (abbreviation: SVM - Support Vector Machines, GP - Gaussian Process)}
\label{regressioncomparison}
\begin{tabular}{|lccccccccc|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Regression   models}}} & \multicolumn{9}{c|}{\textbf{STS configuration}}                                                                                                                                                                                                                                                                                   \\ \cline{2-10} 
\multicolumn{1}{|l|}{}                                              & \multicolumn{1}{c|}{\textbf{STS 1}}    & \multicolumn{1}{c|}{\textbf{STS 2a}}    & \multicolumn{1}{c|}{\textbf{STS 2b}}    & \multicolumn{1}{c|}{\textbf{STS 3a}}    & \multicolumn{1}{c|}{\textbf{STS 3b}}    & \multicolumn{1}{c|}{\textbf{STS 4a}}    & \multicolumn{1}{c|}{\textbf{STS 4b}}   & \multicolumn{1}{c|}{\textbf{STS 4c}}    & \textbf{STS 4d}    \\ \hline

\multicolumn{1}{|l|}{Linear Regression}                                        & \multicolumn{1}{c|}{2.22}          & \multicolumn{1}{c|}{5.98}          & \multicolumn{1}{c|}{7.23}          & \multicolumn{1}{c|}{4.87}          & \multicolumn{1}{c|}{2.85}          & \multicolumn{1}{c|}{7.28}          & \multicolumn{1}{c|}{7.17}         & \multicolumn{1}{c|}{5.91}          & 3.66          \\ 
\multicolumn{1}{|l|}{Interactions Linear Regression}                           & \multicolumn{1}{c|}{1.78}          & \multicolumn{1}{c|}{5.01}          & \multicolumn{1}{c|}{6.45}          & \multicolumn{1}{c|}{3.45}          & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{6.61}          & \multicolumn{1}{c|}{6.102}        & \multicolumn{1}{c|}{5.54}          & 3.13          \\ 
\multicolumn{1}{|l|}{Robust Linear Regression}                                        & \multicolumn{1}{c|}{2.54}          & \multicolumn{1}{c|}{6.33}          & \multicolumn{1}{c|}{7.74}          & \multicolumn{1}{c|}{6.13}          & \multicolumn{1}{c|}{3.81}          & \multicolumn{1}{c|}{9.17}          & \multicolumn{1}{c|}{8.29}         & \multicolumn{1}{c|}{6.72}          & 3.66          \\ 
\multicolumn{1}{|l|}{Stepwise Linear Regression}                               & \multicolumn{1}{c|}{1.78}          & \multicolumn{1}{c|}{5.01}          & \multicolumn{1}{c|}{6.46}          & \multicolumn{1}{c|}{3.46}          & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{6.61}          & \multicolumn{1}{c|}{6.11}         & \multicolumn{1}{c|}{5.54}          & 3.14          \\ \hline

\multicolumn{1}{|l|}{Fine Regression Tree}                                     & \multicolumn{1}{c|}{1.08}          & \multicolumn{1}{c|}{3.19}          & \multicolumn{1}{c|}{4.34}          & \multicolumn{1}{c|}{2.82}          & \multicolumn{1}{c|}{1.31}          & \multicolumn{1}{c|}{4.07}          & \multicolumn{1}{c|}{4.69}         & \multicolumn{1}{c|}{3.27}          & 1.59          \\ 
\multicolumn{1}{|l|}{Medium Regression Tree}                                   & \multicolumn{1}{c|}{1.18}          & \multicolumn{1}{c|}{3.02}          & \multicolumn{1}{c|}{4.26}          & \multicolumn{1}{c|}{2.62}          & \multicolumn{1}{c|}{1.24}          & \multicolumn{1}{c|}{3.86}          & \multicolumn{1}{c|}{4.5}          & \multicolumn{1}{c|}{3.1}           & 1.625         \\
\multicolumn{1}{|l|}{Coarse Regression Tree}                                   & \multicolumn{1}{c|}{1.42}          & \multicolumn{1}{c|}{3.5}           & \multicolumn{1}{c|}{4.52}          & \multicolumn{1}{c|}{2.58}          & \multicolumn{1}{c|}{1.31}          & \multicolumn{1}{c|}{4.2}           & \multicolumn{1}{c|}{4.73}         & \multicolumn{1}{c|}{3.49}          & 1.73          \\ \hline

\multicolumn{1}{|l|}{Linear SVM}                                        & \multicolumn{1}{c|}{2.4}           & \multicolumn{1}{c|}{6.1}           & \multicolumn{1}{c|}{7.52}          & \multicolumn{1}{c|}{5.39}          & \multicolumn{1}{c|}{2.94}          & \multicolumn{1}{c|}{8.09}          & \multicolumn{1}{c|}{7.41}         & \multicolumn{1}{c|}{6.18}          & 3.74          \\ 
\multicolumn{1}{|l|}{Quadratic SVM}                                     & \multicolumn{1}{c|}{1.93}          & \multicolumn{1}{c|}{5.98}          & \multicolumn{1}{c|}{6.96}          & \multicolumn{1}{c|}{3.62}          & \multicolumn{1}{c|}{2.09}          & \multicolumn{1}{c|}{7.98}          & \multicolumn{1}{c|}{5.82}         & \multicolumn{1}{c|}{5.63}          & 2.95          \\ 
\multicolumn{1}{|l|}{Cubic SVM}                                         & \multicolumn{1}{c|}{2.29}          & \multicolumn{1}{c|}{28.81}         & \multicolumn{1}{c|}{12.43}         & \multicolumn{1}{c|}{21.54}         & \multicolumn{1}{c|}{10.02}         & \multicolumn{1}{c|}{17.45}         & \multicolumn{1}{c|}{28.25}        & \multicolumn{1}{c|}{15.23}         & 24.8          \\ 
\multicolumn{1}{|l|}{Fine Gaussian SVM}                                 & \multicolumn{1}{c|}{1.04}          & \multicolumn{1}{c|}{2.42}          & \multicolumn{1}{c|}{4.34}          & \multicolumn{1}{c|}{2.319}         & \multicolumn{1}{c|}{1.3}           & \multicolumn{1}{c|}{3.31}          & \multicolumn{1}{c|}{3.7}          & \multicolumn{1}{c|}{2.95}          & 1.33          \\ 
\multicolumn{1}{|l|}{Medium Gaussian SVM}                               & \multicolumn{1}{c|}{1.24}          & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{4.26}          & \multicolumn{1}{c|}{2.73}          & \multicolumn{1}{c|}{1.52}          & \multicolumn{1}{c|}{3.96}          & \multicolumn{1}{c|}{4.5}          & \multicolumn{1}{c|}{3.98}          & 1.77          \\
\multicolumn{1}{|l|}{Coarse Gaussian SVM}                                & \multicolumn{1}{c|}{1.67}          & \multicolumn{1}{c|}{4.68}          & \multicolumn{1}{c|}{4.52}          & \multicolumn{1}{c|}{3.22}          & \multicolumn{1}{c|}{2}             & \multicolumn{1}{c|}{5.92}          & \multicolumn{1}{c|}{5.68}         & \multicolumn{1}{c|}{5.45}          & 2.78          \\ \hline



\multicolumn{1}{|l|}{Rational Quadratic GP}                            & \multicolumn{1}{c|}{0.72}          & \multicolumn{1}{c|}{\textbf{2.21}} & \multicolumn{1}{c|}{3.4}           & \multicolumn{1}{c|}{2.16}          & \multicolumn{1}{c|}{1.08}          & \multicolumn{1}{c|}{3.34}          & \multicolumn{1}{c|}{3.59}         & \multicolumn{1}{c|}{2.56}          & 1.22          \\
\multicolumn{1}{|l|}{Squared Exponential GP}                           & \multicolumn{1}{c|}{0.87}          & \multicolumn{1}{c|}{2.41}          & \multicolumn{1}{c|}{3.31}          & \multicolumn{1}{c|}{2.25}          & \multicolumn{1}{c|}{1.17}          & \multicolumn{1}{c|}{3.27}          & \multicolumn{1}{c|}{3.65}         & \multicolumn{1}{c|}{2.72}          & 1.26          \\ 
\multicolumn{1}{|l|}{Matern 5/2 GP}                                    & \multicolumn{1}{c|}{0.8}           & \multicolumn{1}{c|}{2.27}          & \multicolumn{1}{c|}{\textbf{3.24}} & \multicolumn{1}{c|}{2.2}           & \multicolumn{1}{c|}{1.14}          & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{3.6}          & \multicolumn{1}{c|}{2.61}          & 1.2           \\ 
\multicolumn{1}{|l|}{Exponential GP}                                   & \multicolumn{1}{c|}{\textbf{0.72}} & \multicolumn{1}{c|}{2.24}          & \multicolumn{1}{c|}{3.35}          & \multicolumn{1}{c|}{\textbf{2.15}} & \multicolumn{1}{c|}{\textbf{1.06}} & \multicolumn{1}{c|}{\textbf{3.25}} & \multicolumn{1}{c|}{\textbf{3.6}} & \multicolumn{1}{c|}{\textbf{2.53}} & \textbf{1.18} \\ \hline

\multicolumn{1}{|l|}{Boosted Ensemble of Trees}                                 & \multicolumn{1}{c|}{1.67}          & \multicolumn{1}{c|}{3.6}           & \multicolumn{1}{c|}{4.6}           & \multicolumn{1}{c|}{2.57}          & \multicolumn{1}{c|}{1.56}          & \multicolumn{1}{c|}{3.88}          & \multicolumn{1}{c|}{4.59}         & \multicolumn{1}{c|}{3.65}          & 1.8           \\ 
\multicolumn{1}{|l|}{Bagged Ensemble of Trees}                                  & \multicolumn{1}{c|}{0.94}          & \multicolumn{1}{c|}{2.63}          & \multicolumn{1}{c|}{3.67}          & \multicolumn{1}{c|}{2.29}          & \multicolumn{1}{c|}{1.08}          & \multicolumn{1}{c|}{3.41}          & \multicolumn{1}{c|}{3.86}         & \multicolumn{1}{c|}{2.62}          & 1.3           \\ \hline

\multicolumn{1}{|l|}{Narrow Neural Network}                                 & \multicolumn{1}{c|}{1.2}           & \multicolumn{1}{c|}{3.48}          & \multicolumn{1}{c|}{5.21}          & \multicolumn{1}{c|}{2.83}          & \multicolumn{1}{c|}{1.47}          & \multicolumn{1}{c|}{4.63}          & \multicolumn{1}{c|}{4.8}          & \multicolumn{1}{c|}{3.86}          & 1.62          \\ 
\multicolumn{1}{|l|}{Medium Neural Network}                                 & \multicolumn{1}{c|}{1.15}          & \multicolumn{1}{c|}{2.88}          & \multicolumn{1}{c|}{4.94}          & \multicolumn{1}{c|}{2.53}          & \multicolumn{1}{c|}{1.49}          & \multicolumn{1}{c|}{3.74}          & \multicolumn{1}{c|}{4.27}         & \multicolumn{1}{c|}{3.305}         & 1.51          \\ 
\multicolumn{1}{|l|}{Wide Neural Network}                           & \multicolumn{1}{c|}{1.05}          & \multicolumn{1}{c|}{2.89}          & \multicolumn{1}{c|}{4.32}          & \multicolumn{1}{c|}{2.35}          & \multicolumn{1}{c|}{1.37}          & \multicolumn{1}{c|}{3.64}          & \multicolumn{1}{c|}{3.85}         & \multicolumn{1}{c|}{2.89}          & 1.34          \\ 
\multicolumn{1}{|l|}{Bilayered Neural Network}                      & \multicolumn{1}{c|}{1.07}          & \multicolumn{1}{c|}{2.68}          & \multicolumn{1}{c|}{5.27}          & \multicolumn{1}{c|}{2.36}          & \multicolumn{1}{c|}{1.29}          & \multicolumn{1}{c|}{3.63}          & \multicolumn{1}{c|}{4.33}         & \multicolumn{1}{c|}{5.13}          & 1.41          \\
\multicolumn{1}{|l|}{Trilayered Neural Network}                     & \multicolumn{1}{c|}{0.9}           & \multicolumn{1}{c|}{2.52}          & \multicolumn{1}{c|}{4.03}          & \multicolumn{1}{c|}{2.28}          & \multicolumn{1}{c|}{1.29}          & \multicolumn{1}{c|}{3.42}          & \multicolumn{1}{c|}{3.95}         & \multicolumn{1}{c|}{2.94}          & 1.31          \\ \hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> parts/table21.tex <==
\begin{table*}[tb!]
\small\addtolength{\tabcolsep}{-4pt}
\centering
\caption{Comparison of various classifier models based on validation accuracy for estimating contact force locations (abbreviation: SVM - Support Vector Machines, K-Nearest Neighbours Algorithm)}
\label{classifiercomparison}
\begin{tabular}{|l|ccccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Classifier   Models}}} & \multicolumn{9}{c|}{\textbf{STS configuration}}                                                                                                                                                                                                                                                                                  \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                              & \multicolumn{1}{c|}{\textbf{STS 1}}    & \multicolumn{1}{c|}{\textbf{STS 2a}}    & \multicolumn{1}{c|}{\textbf{STS 2b}}    & \multicolumn{1}{c|}{\textbf{STS 3a}}    & \multicolumn{1}{c|}{\textbf{STS 3b}}    & \multicolumn{1}{c|}{\textbf{STS 4a}}    & \multicolumn{1}{c|}{\textbf{STS 4b}}    & \multicolumn{1}{c|}{\textbf{STS 4c}}    & \textbf{STS 4d}    \\ \hline

Fine Tree                                                           & \multicolumn{1}{c|}{91.3}          & \multicolumn{1}{c|}{93.2}          & \multicolumn{1}{c|}{95}            & \multicolumn{1}{c|}{90.5}          & \multicolumn{1}{c|}{86.1}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{95.6}          & 93.9          \\ 
Medium Tree                                                         & \multicolumn{1}{c|}{78.8}          & \multicolumn{1}{c|}{92.9}          & \multicolumn{1}{c|}{85.8}          & \multicolumn{1}{c|}{87.6}          & \multicolumn{1}{c|}{74.2}          & \multicolumn{1}{c|}{85.7}          & \multicolumn{1}{c|}{90.1}          & \multicolumn{1}{c|}{94.8}          & 78.5          \\ 
Coarse Tree                                                         & \multicolumn{1}{c|}{69.9}          & \multicolumn{1}{c|}{87.1}          & \multicolumn{1}{c|}{71}            & \multicolumn{1}{c|}{74.5}          & \multicolumn{1}{c|}{60.2}          & \multicolumn{1}{c|}{77.1}          & \multicolumn{1}{c|}{84.2}          & \multicolumn{1}{c|}{87.6}          & 67            \\ \hline

Linear Discriminant                                                 & \multicolumn{1}{c|}{70.7}          & \multicolumn{1}{c|}{89.4}          & \multicolumn{1}{c|}{89.2}          & \multicolumn{1}{c|}{74.8}          & \multicolumn{1}{c|}{59}            & \multicolumn{1}{c|}{79}            & \multicolumn{1}{c|}{82.1}          & \multicolumn{1}{c|}{70.4}          & 73.5          \\ 
Quadratic Discriminant                                              & \multicolumn{1}{c|}{70.3}          & \multicolumn{1}{c|}{89}            & \multicolumn{1}{c|}{89.5}          & \multicolumn{1}{c|}{79}            & \multicolumn{1}{c|}{58.4}          & \multicolumn{1}{c|}{80.6}          & \multicolumn{1}{c|}{88}            & \multicolumn{1}{c|}{88}            & 87.3          \\ \hline
 
Guassian Naïve Bayes                                                & \multicolumn{1}{c|}{42.2}          & \multicolumn{1}{c|}{73.9}          & \multicolumn{1}{c|}{72.7}          & \multicolumn{1}{c|}{46.3}          & \multicolumn{1}{c|}{39.2}          & \multicolumn{1}{c|}{74}            & \multicolumn{1}{c|}{79.2}          & \multicolumn{1}{c|}{63.8}          & 60.9          \\ 
Kernal Naïve Bayes                                                  & \multicolumn{1}{c|}{72.6}          & \multicolumn{1}{c|}{84.2}          & \multicolumn{1}{c|}{78.1}          & \multicolumn{1}{c|}{77.2}          & \multicolumn{1}{c|}{61.9}          & \multicolumn{1}{c|}{77.3}          & \multicolumn{1}{c|}{86.6}          & \multicolumn{1}{c|}{89.7}          & 73.9          \\ \hline

Linear SVM                                                              & \multicolumn{1}{c|}{77.2}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{88.5}          & \multicolumn{1}{c|}{78.4}          & \multicolumn{1}{c|}{62.7}          & \multicolumn{1}{c|}{84.4}          & \multicolumn{1}{c|}{86}            & \multicolumn{1}{c|}{83.4}          & 84.4          \\ 
Quadratic SVM                                                           & \multicolumn{1}{c|}{94.3}          & \multicolumn{1}{c|}{91.9}          & \multicolumn{1}{c|}{93.5}          & \multicolumn{1}{c|}{90.2}          & \multicolumn{1}{c|}{61.1}          & \multicolumn{1}{c|}{88}            & \multicolumn{1}{c|}{93.6}          & \multicolumn{1}{c|}{96.1}          & 89.1          \\ 
Cubic SVM                                                               & \multicolumn{1}{c|}{72}            & \multicolumn{1}{c|}{65.9}          & \multicolumn{1}{c|}{95.7}          & \multicolumn{1}{c|}{48.2}          & \multicolumn{1}{c|}{53.2}          & \multicolumn{1}{c|}{64.5}          & \multicolumn{1}{c|}{60.8}          & \multicolumn{1}{c|}{71.8}          & 74.9          \\ 
Fine Guassian SVM                                                       & \multicolumn{1}{c|}{96}            & \multicolumn{1}{c|}{\textbf{95.7}} & \multicolumn{1}{c|}{98.1}          & \multicolumn{1}{c|}{92.2}          & \multicolumn{1}{c|}{87.8}          & \multicolumn{1}{c|}{92.6}          & \multicolumn{1}{c|}{\textbf{95.4}} & \multicolumn{1}{c|}{97.2}          & 97.1          \\
Medium Guassian SVM                                                   & \multicolumn{1}{c|}{94.4}          & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{93}            & \multicolumn{1}{c|}{91.3}          & \multicolumn{1}{c|}{81.3}          & \multicolumn{1}{c|}{91.2}          & \multicolumn{1}{c|}{93.8}          & \multicolumn{1}{c|}{95.9}          & 93.2          \\ 
Coarse Guassian SVM                                                    & \multicolumn{1}{c|}{74.4}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{88.7}          & \multicolumn{1}{c|}{88.5}          & \multicolumn{1}{c|}{63.9}          & \multicolumn{1}{c|}{85.6}          & \multicolumn{1}{c|}{89.1}          & \multicolumn{1}{c|}{86.8}          & 87.5          \\ \hline

Fine KNN                                                            & \multicolumn{1}{c|}{95}            & \multicolumn{1}{c|}{94.5}          & \multicolumn{1}{c|}{97.7}          & \multicolumn{1}{c|}{90.2}          & \multicolumn{1}{c|}{89.3}          & \multicolumn{1}{c|}{91.2}          & \multicolumn{1}{c|}{93.7}          & \multicolumn{1}{c|}{96.6}          & 96.6          \\ 
Medium KNN                                                          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{95.4}          & \multicolumn{1}{c|}{98}            & \multicolumn{1}{c|}{92.1}          & \multicolumn{1}{c|}{91}            & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{97}            & 97.3          \\ 
Coarse KNN                                                          & \multicolumn{1}{c|}{82.7}          & \multicolumn{1}{c|}{93.4}          & \multicolumn{1}{c|}{93.4}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{81}            & \multicolumn{1}{c|}{91.1}          & \multicolumn{1}{c|}{93.2}          & \multicolumn{1}{c|}{93.6}          & 92.7          \\ 
Cosine KNN                                                          & \multicolumn{1}{c|}{86.6}          & \multicolumn{1}{c|}{93.7}          & \multicolumn{1}{c|}{95.5}          & \multicolumn{1}{c|}{90}            & \multicolumn{1}{c|}{85.3}          & \multicolumn{1}{c|}{89.4}          & \multicolumn{1}{c|}{92.6}          & \multicolumn{1}{c|}{89.2}          & 90.7          \\ 
Cubic KNN                                                           & \multicolumn{1}{c|}{94.4}          & \multicolumn{1}{c|}{95.3}          & \multicolumn{1}{c|}{98}            & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{90.6}          & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{97}            & 97.2          \\ 
Weighted KNN                                                        & \multicolumn{1}{c|}{95.8}          & \multicolumn{1}{c|}{95.6}          & \multicolumn{1}{c|}{\textbf{98.2}} & \multicolumn{1}{c|}{92.1}          & \multicolumn{1}{c|}{91}            & \multicolumn{1}{c|}{\textbf{92.8}} & \multicolumn{1}{c|}{94.8}          & \multicolumn{1}{c|}{\textbf{97.2}} & \textbf{97.3} \\ \hline

Boosted Ensemble Trees                                                       & \multicolumn{1}{c|}{82.7}          & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{90.4}          & \multicolumn{1}{c|}{75.8}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{96}            & 91.1          \\ 
Bagged Ensemble Trees                                                        & \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{95.4}          & \multicolumn{1}{c|}{97.6}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{\textbf{91.9}} & \multicolumn{1}{c|}{92.6}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{96.9}          & 96.8          \\ 
Subspace Discriminant                                               & \multicolumn{1}{c|}{50.9}          & \multicolumn{1}{c|}{78.4}          & \multicolumn{1}{c|}{85.3}          & \multicolumn{1}{c|}{60.8}          & \multicolumn{1}{c|}{49.7}          & \multicolumn{1}{c|}{75.4}          & \multicolumn{1}{c|}{84.1}          & \multicolumn{1}{c|}{66.9}          & 74.1          \\ 
Subspace Ensemble KNN                                                        & \multicolumn{1}{c|}{89.7}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{90}            & \multicolumn{1}{c|}{84.1}          & \multicolumn{1}{c|}{82.1}          & \multicolumn{1}{c|}{85.4}          & \multicolumn{1}{c|}{86}            & \multicolumn{1}{c|}{92.7}          & 91.4          \\ 
RUSBossted Ensemble Trees                                                    & \multicolumn{1}{c|}{78.8}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{85.8}          & \multicolumn{1}{c|}{87.6}          & \multicolumn{1}{c|}{74.2}          & \multicolumn{1}{c|}{85.7}          & \multicolumn{1}{c|}{90.1}          & \multicolumn{1}{c|}{94.9}          & 78.5          \\  \hline

Narrow Neural Network                                                           & \multicolumn{1}{c|}{95.6}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{96.9}          & \multicolumn{1}{c|}{91.7}          & \multicolumn{1}{c|}{86.7}          & \multicolumn{1}{c|}{92.2}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{96.9}          & 95.8          \\ 
Medium Neural Network                                                           & \multicolumn{1}{c|}{96.3}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{97.8}          & \multicolumn{1}{c|}{92.3}          & \multicolumn{1}{c|}{89.4}          & \multicolumn{1}{c|}{92.5}          & \multicolumn{1}{c|}{95.3}          & \multicolumn{1}{c|}{97.1}          & 97.2          \\ 
Wide Neural Network                                                             & \multicolumn{1}{c|}{96.1}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{97.6}          & \multicolumn{1}{c|}{92.2}          & \multicolumn{1}{c|}{90.3}          & \multicolumn{1}{c|}{92.5}          & \multicolumn{1}{c|}{94}            & \multicolumn{1}{c|}{97}            & 96.8          \\ 
Bilayered Neural Network                                                        & \multicolumn{1}{c|}{96.2}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{97.2}          & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{89}            & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{96.9}          & 96.9          \\ 
Trilayered Neural Network                                                       & \multicolumn{1}{c|}{95.8}          & \multicolumn{1}{c|}{95.1}          & \multicolumn{1}{c|}{97.6}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{89.3}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{94.5}          & \multicolumn{1}{c|}{97.2}          & 97            \\ \hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> parts/table3.tex <==
\begin{table*}[t!]
\centering
\small\addtolength{\tabcolsep}{-4pt}
\caption{ Estimating the location of contact force for 170 test cases for  points A, B, C as shown in Fig.~\ref{points}}
\label{contactprediction}
\begin{tabular}{|c|ccccccccc|}

\hline
\multirow{2}{*}{\textbf{True predictions}} & \multicolumn{9}{c|}{\textbf{STS configuration}}                                                                                                                                                                                                                                       \\ \cline{2-10} 
                     & \multicolumn{1}{c|}{STS 1}    & \multicolumn{1}{c|}{STS 2a}    & \multicolumn{1}{c|}{STS 2b}    & \multicolumn{1}{c|}{STS 3a}    & \multicolumn{1}{c|}{STS 3b}    & \multicolumn{1}{c|}{STS 4a}    & \multicolumn{1}{c|}{STS 4b}    & \multicolumn{1}{c|}{STS 4c}    & \multicolumn{1}{c|}{STS 4d} \\ \hline
A                    & \multicolumn{1}{c|}{169}   & \multicolumn{1}{c|}{169}   & \multicolumn{1}{c|}{168}   & \multicolumn{1}{c|}{165}   & \multicolumn{1}{c|}{163}   & \multicolumn{1}{c|}{168}   & \multicolumn{1}{c|}{168}   & \multicolumn{1}{c|}{168}   & 168   \\ \hline
B                   & \multicolumn{1}{c|}{160}   & \multicolumn{1}{c|}{168}   & \multicolumn{1}{c|}{169}   & \multicolumn{1}{c|}{150}   & \multicolumn{1}{c|}{142}   & \multicolumn{1}{c|}{151}   & \multicolumn{1}{c|}{156}   & \multicolumn{1}{c|}{165}   & 167   \\ \hline
C                   & \multicolumn{1}{c|}{164}   & \multicolumn{1}{c|}{153}   & \multicolumn{1}{c|}{168}   & \multicolumn{1}{c|}{161}   & \multicolumn{1}{c|}{150}   & \multicolumn{1}{c|}{155}   & \multicolumn{1}{c|}{162}   & \multicolumn{1}{c|}{166}   & 162   \\ \hline    
\textbf{Accuracy} (\%)                    & \multicolumn{1}{c|}{96.66} & \multicolumn{1}{c|}{96.07} & \multicolumn{1}{c|}{99.01} & \multicolumn{1}{c|}{93.33} & \multicolumn{1}{c|}{89.21} & \multicolumn{1}{c|}{92.94} & \multicolumn{1}{c|}{95.29} & \multicolumn{1}{c|}{97.84} & 97.45 \\ \hline
\end{tabular}
\end{table*}

